DMPlug: A Plug-in Method for Solving Inverse Problems with Diffusion Models

Pretrained diffusion models (DMs) have recently been popularly used in solving inverse problems (IPs). The existing methods mostly interleave iterative steps in the reverse diffusion process and iterative steps to bring the iterates closer to satisfying the measurement constraint. However, such interleaving methods struggle to produce final results that look like natural objects of interest (i.e., manifold feasibility) and fit the measurement (i.e., measurement feasibility), especially for nonlinear IPs. Moreover, their capabilities to deal with noisy IPs with unknown types and levels of measurement noise are unknown. In this paper, we advocate viewing the reverse process in DMs as a function and propose a novel plug-in method for solving IPs using pretrained DMs, dubbed DMPlug. DMPlug addresses the issues of manifold feasibility and measurement feasibility in a principled manner, and also shows great potential for being robust to unknown types and levels of noise. Through extensive experiments across various IP tasks, including two linear and three nonlinear IPs, we demonstrate that DMPlug consistently outperforms state-of-the-art methods, often by large margins especially for nonlinear IPs. The code is available at https://github.com/sun-umn/DMPlug.

==> sections/sec3_method_old.tex <==
\section{Method}
\label{sec:method}

\subsection{Proposed method}
\label{subsec:method}

To avoid the insufficient feasibility issue of the current interleaving methods, we propose a novel method that encodes the prior information of pre-trained DMs into the conventional MAP framework instead of interleaving different processes, and promotes data consistency by directly minimizing the residual term $||\mb y - \mc{A}\paren{\mb x}||$. The main idea consists of \textbf{(1) viewing the reverse diffusion process $\mc R$ as a function} which contains multiple reverse steps and maps from the seed space to the image manifold; \textbf{(2) parameterizing the image as $\mb x = \mc R\paren{\mb z}$ and pluging it into \cref{eq:MAP}} to form a unified optimization formulation for solving numerous IPs. In this work, we drop the explicit regularizer $\mc{\phi}\paren{\cdot}$ and use instead the prior captured by pre-trained DMs. The final formulation of our method arrives at

\begin{align} \label{eq:ours}
    \mb z^* = \argmin_{\mb z}\; \ell\paren{\mb y, \mc{A}\paren{\mc R\paren{\mb z}}}, \quad \quad \mb x^* = \mc{R}\paren{\mb z^*},
\end{align}

where $\ell\paren{\cdot}$ is a distance metric such as \textit{Mean Square Error (MSE)}, $\mc R\paren{\cdot}$ is the \textit{fixed} and \textit{pre-trained} reverse diffusion process, and $\mb z$ is a trainable seed. The (local) minimizer $\mb z^*$ can be solved by using an optimizer such as gradient descent, starting from a random initialization. Given the resulting (local) minimizer $\mb z^*$, the reconstructed image is obtained as $\mb x^* = \mc{R}\paren{\mb z^*}$. With proper solution to the optimization problem in \cref{eq:ours}, the reconstructed image $\mb x^*$ is expected to \textbf{exhibit realism}, attributed to the pre-trained DM $\mc{R}\paren{\cdot}$, while also \textbf{satisfying data consistency requirements}, i.e., $\mb y \approx \mc{A} \paren{\mb x^*}$.

\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/psnrvstime1.png}
    \caption{\textbf{PSNR (dB) vs. per-iteration wall-clock time (second)} running on an \textit{NVIDIA A100}, for various number of reverse steps in $\mc{R}$. Experiments are conducted on $50$ cases from \textbf{CelebA}~\cite{liu_deep_2015} for the $4 \times$ super-resolution task.}
    \label{fig:psnrvstime1}
\end{wrapfigure}

However, considering that DMs typically require dozens or hundreds of sampling steps for high-quality image generation~\cite{ho_denoising_2020,song_denoising_2022,rombach_high-resolution_2022}, both the memory costs and the computational complexity of the proposed algorithm can appear to be exceedingly high. This is because each gradient update in the proposed algorithm requires a full forward and backward pass through the entire diffusion process. To remedy this, we use DDIM, which allows for skipping sampling steps thanks to its non-Markovian property, as the sampler for the reverse process $\mc{R}$, and further decrease the number of reverse steps in $\mc{R}$ based on \textbf{two essential phenomenons}. We conduct example experiments on CelebA for super-resolution to show the trend of PSNR vs. per-iteration wall-clock time with the changes of the number of reverse steps, as shown in \cref{fig:psnrvstime1}. \textbf{Phenomenon (1):} merely employing a few reverse steps, such as $2$ and $3$, are sufficient for the proposed method to address IPs, contrary to the requirements typically associated with image generation. The reason may be that the measurement $\mb y$ compensates part of prior information for solving \cref{eq:ours}. \textbf{Phenomenon (2):} the fewer reverse steps in $\mc{R}$ can lead to better reconstruction performance and lower computational costs, which is opposite with the image generation cases. We speculate that adding more reverse steps likely increases the non-convexity of the optimization problem in \cref{eq:ours}, thereby making it more challenging to find an optimal solution. \cref{fig:psnrvstime2} shows the similar trend for PSNR vs. wall-clock time to reach peaks.


\begin{figure*}[!htbp]
    \centering 
    % \vspace{-1em}
    \includegraphics[width=0.95\linewidth]{figures/regression_denoising.png}
    % \vspace{-1em}
    \caption{(1): Evolution of \textbf{image regression} using different target images. (2): The ``early-learning-then-overfitting'' (ELTO) phenomenon in the proposed method for \textbf{image denoising}. The quality of the estimated image climbs first to the peak and then drops once the noise is picked up by the model $\mc{R}\paren{\mb z}$. The detection of ES-WMV~\cite{wang_early_2023} relies on the variance curve, whose valley is often well aligned with the PSNR peak.}
    \label{fig:regression_denoising}
    % % \vspace{-1em}
\end{figure*} 

\subsection{High resistance to noise}
\label{subsec:resistance}

One may wonder why the frozen and pre-trained DMs with only a few (even $2$ and $3$) reverse steps can be used as an image prior at all. It may seem plausible to find a suitable $\Tilde{\mb z}$ recovering any possible image $\mb x$, even for random noise, as $\mc{R}\paren{\Tilde{\mb z}}$, thereby suggesting that the pre-trained DMs do not impose any constraints on the generated image. Here, we would like to show that although the proposed method can fit nearly any image, it seems to resist "undesirable" outcomes and converge much faster towards desired visual content based on several toy experiments below.

\paragraph{\textcolor{umn_maroon}{Image regression}} First, we attempt to use our method \cref{eq:ours} to fit different images. Given a target image $\mb x_0$, the image regression task aims to find an appropriate $\mb z$ that can reproduce $\mb x_0$, which can be formulated as $\min_{\mb z}\; \ell\paren{\mb x_0, \mc R\paren{\mb z}}$. In \cref{fig:regression_denoising} (1), we choose the \textit{MSE} loss as $\ell\paren{\cdot}$ and \textit{ADAM} with the same learning rate $0.01$ as the optimizer to fit three different choices for $\mb x_0$: (a) a natural image, (b) the same image after randomly shuffling the pixels, (c) and random noise sampled from $\mc{U}\paren{0, 1}$. The figure clearly indicates that although the proposed method can even fit random noise, the convergence speed of the case (a) is much faster than cases (b) and (c). In other words, the proposed method exhibits a high resistance to noise and a low resistance to signal.

\paragraph{\textcolor{umn_maroon}{Image denoising}} The above experiment only shows the convergence pattern of fitting different images alone. Then one may wonder whether this good property exists when encountering both signal and undesirable components together. Given a noisy image $\mb y_0 = \mb x_0 + \mb n$, where $\mb n$ is the measurement noise, the image denoising task targets for a suitable $\mb z$ that can recover the image $\mb x_0$. Similarly, we can consider this problem as $\min_{\mb z}\; \ell\paren{\mb y_0, \mc R\paren{\mb z}}$, and use the \textit{MSE} loss as $\ell\paren{\cdot}$ and \textit{ADAM} with the same learning rate $0.01$ as the optimizer. For $\mb n$, we assume it as the common Gaussian noise with $\sigma = 0.08$. By reflecting on the preceding experiment, we can envision that the global optimization would lead to $\mb y_0 = \mc{R}\paren{\mb z}$ instead of $\mb x_0$, as confirmed in \cref{fig:regression_denoising} (2). Fortunately, we observe that the proposed method and first-order optimization methods together offer a blessing: $\mc{R}\paren{\mb z}$ has a bias towards the desired visual content and learns it much faster than learning noise. Therefore, the quality of reconstruction climbs to a peak before the potential degradation due to noise. By the way, the “early-learning-then-overfitting” (ELTO) phenomenon has been repeatedly reported in another famous zero-shot IP solver---deep image prior(DIP)~\cite{ulyanov_deep_2020,li_self-validation_2021,li_deep_2023,shi_measuring_2021,wang_early_2023}. With this favorable property and appropriately stopping the optimization process, the proposed method can reconstruct the image $\mb x_0$ even when facing additional measurement noise $\mb n$.

\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/SB.png}
    \caption{The spectral bias of the proposed method.}
    \label{fig:SB}
\end{wrapfigure}

\subsection{Spectral bias}\label{subsec:SB}
% \paragraph{\textcolor{umn_maroon}{Spectral bias}} 

In the denoising experiment above, we observe that the proposed method exhibits a spectral bias during optimization, where the low-frequency components of the target images are learned better and faster compared to the high-frequency components~\cite{chakrabarty_spectral_2019,shi_measuring_2021}. To measure the spectral bias, following~\cite{li_deep_2023,zhuang_blind_2024}, we use the metric dubbed \textit{frequency band error (FBE)}, which calculates the point-wise relative estimation error over the Fourier domain, i.e., $\abs*{\mc F(\mb y) - \mc F(\wh{\mb x})}/\abs*{\mc F(\mb y)}$ where $\mb y$ is the measurement and $\wh{\mb x}$ is the reconstructed image. Then we divide the Fourier frequencies into five bands, compute the per-band average FBE, and show the evolution of all the frequency bands in \cref{fig:SB}. We can clearly find that the low-frequency components are captured much faster than the high-frequency ones. 

It is widely acknowledged that the power spectrum of a natural image decays rapidly from low frequencies to high frequencies~\cite{ruderman_statistics_1994}. Consequently, when the noise level is low, high frequencies are typically dominated by noise, while lower frequencies are more prominently occupied by the natural signal. In this sense, the spectral bias shown in \cref{fig:SB} can also be interpreted as an ELTO phenomenon from the frequency perspective.

\subsection{Beyond non-blind IPs}\label{subsec:non_blind}

The proposed method in \cref{subsec:method} considers non-blind IPs, i.e., when the forward operator $\mc{A}\paren{\cdot}$ is known, and exhibits SOTA performance for these applications, as shown in \cref{tab:sr_inp,tab:sr_inp_bedroom,tab:NBID}. In this section, we would like to demonstrate the flexibility of our method by adapting the proposed to some blind applications, including BID and BID with turbulence.

\begin{align} \label{eq:MAP_BID}
    \min_{\mb z,\mb b} \hspace{0.25em} \ell \Big(\mb y, \hspace{0.25em} \underbrace{\textit{SoftMax}\paren{\mb b}}_{\text{Kernel rec.}} \ast  \underbrace{\mathcal{R} \paren{\mb z}}_{\text{Image rec.}} \Big), \quad \text{(for \textbf{BID)}}
\end{align}

\begin{align} \label{eq:MAP_turbulence}
    \min_{\mb z,\mb b,\mb \phi} \hspace{0.25em} \ell \Big(\mb y, \hspace{0.25em} \underbrace{\textit{SoftMax}\paren{\mb b}}_{\text{Kernel rec.}} \ast  \mathcal{T}_{\mb \phi}(\underbrace{\mathcal{R} \paren{\mb z}}_{\text{Image rec.}}) \Big), \quad \text{(for \textbf{turbulence)}}
\end{align}



\subsection{Seemingly similar ideas}\label{subsec:similar}

\paragraph{\textcolor{umn_maroon}{GAN-inversion}} 

The image recovery part of our method, i.e., $\mathcal{R} \paren{\mb z}$, is reminiscent of the classical GAN-inversion~\cite{creswell_inverting_2016,zhu_generative_2018}. To recover a clean image $\mb x$ from the measurement $\mb y \approx \mc A(\mb x)$, existing GAN-inversion methods typically first solve $\mb e^* = \arg\min_{\mb e} \ell(\mb y, \mc A \paren {\mc G_{\mb \beta} \paren{\mb e}}$, where $\mc G$ is a pre-trained GAN generator parameterized by $\mb \beta$ and $\mb e$ is the latent code, and then reconstructed image is represented as $\mc G_{\mb \beta} \paren {\mb e^*}$. There are some following works that make the generator $\mc G$ trainable as well~\cite{pan_exploiting_2020}. Both the proposed method and GAN-inversion aim to find an appropriate latent vector which can satisfy the data consistency, whereas DMs tend to generate higher-quality images~\cite{dhariwal_diffusion_2021} and are free from \textit{mode collapse}~\cite{dhariwal_diffusion_2021,bayat_study_2023}, where the generator simply memorizes several training examples to fool the discriminator~\cite{saatchi_bayesian_2017,zhang_convergence_2018}.

\paragraph{\textcolor{umn_maroon}{Algorithm unrolling}}


\paragraph{\textcolor{umn_maroon}{Diffusion inversion}}
